Elmo: Source-Routed Multicast for Cloud Services

We present Elmo, a system that addresses the multicast scalability problem in multi-tenant data centers. Modern cloud applications frequently exhibit one-to-many communication patterns and, at the same time, require sub-millisecond latencies and high throughput. IP multicast can achieve these requirements but has control- and data-plane scalability limitations that make it challenging to offer it as a service for hundreds of thousands of tenants, typical of cloud environments. Tenants, therefore, must rely on unicast-based approaches (e.g., application-layer or overlay-based) to support multicast in their applications, imposing overhead on throughput and end host CPU utilization, with higher and unpredictable latencies. Elmo scales network multicast by taking advantage of emerging programmable switches and the unique characteristics of data-center networks; specifically, the symmetric topology and short paths in a data center. Elmo encodes multicast group information inside packets themselves, reducing the need to store the same information in network switches. In a three-tier data-center topology with 27K hosts, Elmo supports a million multicast groups using a 325-byte packet header, requiring as few as 1.1K multicast group-table entries on average in leaf switches, with a traffic overhead as low as 5% over ideal multicast.

==> background.tex <==
\section{Background}\label{sec:background}

\ms{merge this with the intro and the design section.}

\subsection{Data Center Networks}
\label{sec:data_center_networks}

Server-to-server traffic~\cite{} dominates modern data-center workloads, hence,
network latency and throughput are a significant factor. Data center networks
are built using multi-rooted Clos or Fat-tree topologies (\eg, Google Fat-Tree
Topology~\cite{}, Facebook Fabric~\cite{}, Brocade's Multi- Fabric
Topology~\cite{}, and Big Switch Cloud Fabric Topology~\cite{}) to provide
scalable throughput in a uniform and predictable manner. These topologies are
designed to provide high bisection bandwidth and predictable latency; and have
a relatively fixed, symmetrical, and modular structure. The path stretch is
also bounded; each host is reachable via other hosts, using a fixed (small)
number of hops. For example, in a two-tier spine leaf topology~\cite{}, each
host is at most three-hops away from other hosts. In these topologies, upstream
traffic is multi-pathed across all available links, and downstream traffic is
routed using route information. In case of link failures, upstream links are
taken out of multipath selection, and packets traverse over remaining
links.

In this paper, we evaluate \name{} using Facebook Fabric Topology. However, our
design applies to all other multi-rooted tree topologies.

In Facebook Fabric Topology, a server-pod is a basic unit of the topology
having four fabric (or spine) switches, each connected to all 48 ToR (leaf)
switches. Each ToR switch can have up to 48 hosts. A server-pod can, therefore,
have a maximum of 2,304 servers. Multiple server-pods are connected using
another set of switches, called plane (or super-spine) switches. Each fabric
switch, of a server-pod, connects to a plane switch, as shown in
Figure~\ref{fig:fb-topology}. The maximum path stretch of Facebook Fabric
Topology is five hops.

%\begin{figure}[t!]
%\centering  
%\includegraphics[width=0.9\linewidth]{figures/FBNetwork.png}  
%\caption{Facebook Fabric Topology (placeholder). \textit{Replace this with a
%figure showing the symmetry and placement (denseness and sparseness) of group
%member VMs under pod/leaf switches of a data center network.}}
%\label{fig:fb-topology}
%\end{figure}

\subsection{Programmable Data Planes}

\ms{this is now moved to Section 5.1.}

Programmable data planes allow for parse, match, and action on custom packet
headers and more. Their behavior is expressed in a high-level domain-specific
language, like P4, and compiles to a software or hardware target. 

In this section, we describe three essential characteristics of these
programmable data planes that we used in building \name{}.

\paragraph{Match-and-set inside parser} Along with parsing headers, parsers in
programmable switches can set custom metadata at each stage of the parser.
Hence, instead of using flow tables, the switch can perform basic match-and-set
operations inside parser. In \name{}, we use this property of the parser to
extract a bitmap among a set of bitmaps inside a \name{} header without using
flow rules. We compare the cost of using flow rules versus match-and-set inside
parser in Section~\ref{}.?

\paragraph{Adding extensions} New extensions can be added to programmable
switches and exposed to the programmer through data-plane languages like P4.
For example, $P4_{16}$ provides support for adding new features via the
\verb|extern| construct. We use this construct to add a new primitive in P4 to
switch packets to an output port(s) using a bitmap. We describe the details of
this primitive in Section~\ref{}, and the associated chip (area, power, and
delay) cost in Section~\ref{}.   

\iffalse
\ms{Here are some Google Patent discussing how current switches map multicast
group id to bit vectors - \\
https://www.google.ch/patents/US20030174725,\\
https://www.google.com/patents/US20040202164. Chapter 11.11 of this book,
https://goo.gl/c63BsA, also discusses the internal workings of multicast and
use of bit vectors.}
\ms{Folks at Barefoot are looking into adding this bitmap-based port select
feature in their next series of switches -- private communication.}
\fi

\paragraph{Arbitrary encapsulation and decapsulation}
In \name{}, we use a software programmable switch (like PISCES) as a hypervisor
switch to encapsulate \name{} header on a packet. Similarly, using hardware
programmable switches, we decapsulate the read bitmaps as the \name{} packets
traverses through the network. \ms{needs better explanation/wording.}



==> motivation.tex <==
\section{Motivation}\label{sec:motivation}

\ms{merge with intro?}

To motivate the need for \name{}, we first highlight the recent changes in data
center workloads, where traffic has shifted from (80\%) north-to-south to
(70\%) east-to-west~\cite{}, giving rise to more complex communication patterns
involving nodes to share identical data to many nodes. We then discuss the
limitations of traditional IP multicast, and how it cannot scale to the number
of groups required by these workloads.

\subsection{Emerging Workloads}

\ms{Rename this section, and discuss how multicast is done right now in the
data center.}
\todo{should we try to taxonomize these different types of multicast workloads?
\eg, provider services or tenant applications etc. needing multicast.}

Several data-center workloads have high request fanout patterns that motivate
the need for in-network multicast.

In streaming telemetry workloads, hosts continuously send telemetry data in
incremental updates to a set of collectors. The collectors use streaming
analytics to infer insights from the incoming data. Similarly, several
data-center applications are designed as feedback-based control loops. Examples
include schedulers and load balancers that require a steady-stream of telemetry
information about the load on servers to make effective server selection
decisions \ls{cite}. In virtualized network environments, overlay multicast and
broadcast between virtual machines of a tenant also stand to benefit from
efficient multicast implementations. Lastly, publish-subscribe systems are
common building blocks for large-scale systems today \ls{give examples}. These
systems create a large number of publish-subscribe topics per user (\ls{cite
the fact that Google gives up to 10K of this per project}).

In the absence of multicast support from cloud providers today (\ls{cite lack
of multicast support in cloud environments}), the above mentioned workloads use
unicast and application overlays instead. For a $1-to-N$ request pattern, the
network and CPU utilization is thereby inflated by $O(N)$. 

Figure~\ref{fig:pubsub-heatmap} shows the physical CPU utilization when a
single ZeroMQ broker\ls{cite} pushes messages from multiple publishers to
multiple subscribers. We vary the number of publishers and subscribers between
1 and 128, in powers of 2. Each publisher issues requests at a rate of 1,000
per second. Four publishers saturate a physical CPU core at the broker when
there are 128 subscribers. With multicast, the CPU utilization at the broker is
instead independent of the number of subscribers (\ls{is the experiment in the
evaluation done with the same settings?} \ms{yes.}). A similar opportunity for
reducing utilization holds within the network as well, details of which appear
in Section~\ref{sec:evaluation}.

\ms{Following paper confirms the degradation in throughput at the virtual
switches when used in an overlay setting to replicate packets across multiple
ports. Paper~\href{http://iqua.ece.toronto.edu/papers/rzhu-infocom17.pdf}
{rzhu-infocom17.pdf}}

\iffalse
% ********** comment start ***********
\ms{Some notes from Lalith:
https://cloud.google.com/pubsub/quotas\#other\_limits. 10K topics per project
are the quota they set for google pub-sub. If you think of a project as a
tenant, 100 tenants already bring us to 1M topics! We could envision 100K per
tenant maybe?  A funny feedback request:
https://googlecloudplatform.uservoice.com/forums/302631-cloud-pub-sub
/suggestions/18828355-remove-topic-limit.}
% ********** comment end ***********
\fi

%\begin{figure}[t!]
%\centering  
%\includegraphics[width=0.9\linewidth]{figures/pubsub-heatmap.pdf}  
%\caption{A heat map of a single-core physical CPU utilization for varying
%number of publishers and subscribers.}
%\label{fig:pubsub-heatmap}
%\end{figure}

\subsection{Limitations of IP Multicast}
Historically, decentralized IP multicast protocols have been difficult to scale
to large group sizes given the lack of stability and hardware limitations
\ls{DCN paper and Citation 11 from DCN} paper. In particular, protocols such as
IGMP and PIM trigger many control messages during churn, need to query the
entire broadcast domain periodically, and are not robust to network failures.
The number of multicast groups a single switch could support were also limited
\ls{numbers from DCN paper}.

SDN-based multicast overcame the control plane obstacles posed by IGMP and PIM.
With SDN, a logically centralized controller installs multicast flow table
rules on forwarding devices. However, a key scalability challenge remains in
the form of the limited number of multicast flow table rules that can be
supported per switch.

Multicast IP addresses are not aggregated like unicast IP prefixes. This
requires a switch to support as many flow table entries as there are multicast
groups it needs to forward. However, hardware limitations on switches today
pose a barrier to this approach. The
RMT~\cite{Bosshart:2013:FMF:2486001.2486011} proposal (on which the Barefoot
Tofino chip is based) provides a total of 46.25MB of SRAM and 5MB for the TCAM
across all 32 stages. Assuming a data center where a spine switch connects to
48 leaves \ls{cite facebook architecture}, a multicast flow rule requires 4
bytes for an IP address and 8 bytes to represent 48 output ports. This
translates to 11MB at every spine switch to support a million multicast groups
in a data-center, representing 25\% of SRAM and more than 2x the TCAM capacity.
Note, this assumes that all the SRAM and TCAM on a switch is available for
hosting multicast entries, which is not the case. In practice, there are
constraints on how these memory blocks can be merged together in the chip.
\ls{@Shahbaz: clarify/cite. The "Compiling Packet Programs to Reconfigurable
Switches" paper from NSDI'15 talks about this in detail}.

Note, the memory and TCAM sizes on the Barefoot Tofino chip are high relative
to other alternatives. The Intel FM6000 chip, for instance, contains 108KB of
memory (\ls{@Shahbaz: SRAM or TCAM?}). High-end Arista and Cisco switches
support only up to 64K multicast groups on their ASIC\ls{@Shahbaz,
cite/confirm}.

Proposals exist to reduce flow table usage via aggregation and compression
\cite{Li:2013:SIM:2535372.2535380}. These approaches trade-off the use of fewer
flow table entries by increasing the traffic overhead: more output ports than
were necessary to emit the same packets.


